A Dataset for Physical and Abstract Plausibility and Sources of Human Disagreement

We present a novel dataset for physical and abstract plausibility of events in English. Based on naturally occurring sentences extracted from Wikipedia, we infiltrate degrees of abstractness, and automatically generate perturbed pseudo-implausible events. We annotate a filtered and balanced subset for plausibility using crowd-sourcing, and perform extensive cleansing to ensure annotation quality. In-depth quantitative analyses indicate that annotators favor plausibility over implausibility and disagree more on implausible events. Furthermore, our plausibility dataset is the first to capture abstractness in events to the same extent as concreteness, and we find that event abstractness has an impact on plausibility ratings: more concrete event participants trigger a perception of implausibility.

==> sections/backup_analysis_of_human_judgements.tex <==
\section{Analysis of Human Judgements} \label{sec:human_analysis}

% @me: disagreement with original label von disagreement among annotators klarer herausarbeiten

\subsection{Examining Rating Distributions}
%\paragraph{Rating Distributions and What They Imply}
Fig.~\ref{fig:rating_insights}(a) shows the distribution of ratings across the four rating options with red and blue bars indicating originally plausible and implausible label. The distribution is skewed towards plausibility with 69.24\% ratings $\in \{4,5\}$. We aggregate all individual ratings as average median rating per triple and show the resulting distribution in Fig.~\ref{fig:rating_insights}(b). While the distribution for originally plausible triples (red bars) evens out as expected with a peak number of average median rating for average plausibility (avg. median ratings $\in \{4\geq3\}$), a similar peak can be observed given the distribution for originally implausibly triples (blue bars). The graph also shows differences, namely substantially more triples with a median rating indicating weak implausibility for originally implausible triples, as well as 76\% more triples with median ratings indicating high plausibility. Moreover, average median ratings for originally plausible triples fall below 2 only in 5 cases, which is the case for 22 originally implausible triples. Lastly, there are 2 triples which are rated unanimously plausible, \textit{candidate-show-ability} and \textit{installation-provide-interpretation}. 

To further investigate the skew towards plausibility, we visualize the average median rating for originally plausible (a) and implausible (b) triples in Fig.~\ref{fig:mean_rating}. The plot also illustrates the standard deviation of the values as a cloud. We observe that annotators tend to show more agreement for plausible triples with standard deviation decreasing with higher plausibility. In contrast, rating triples labeled as implausible results in greater deviation from the average mean rating decreasing only with implausibility. Taking into account the black horizontal line at a median rating of 3, we clearly see that median ratings for originally plausible triples are mostly above the cut line indicating \textit{agreement} with the original label. On the other hand, median ratings for originally implausible triples are mostly below the cut line indicating \textit{disagreement} with the original label.

These observations indicate (i) the tendency that \textbf{humans favor plausibility over implausibility}, while, however, avoiding the extreme on the plausibility end of the scale, and (ii) that \textbf{(potential) implausibility yields higher disagreement} as annotators disagree more when rating triples that were originally labeled as implausible. 

%As the process of automatically generating implausible triples based off attested plausible triples possibly induces plausibility, we perform the following evaluation study. 

\begin{figure*}[!htpb]
     \centering

     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/majority-labels-plausible-hard-maj.png}
         \caption{Attested plausible triples.}
         \label{fig:distribution_plausible_ts}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/majority-labels-implausible-hard-maj.png}
         \caption{Perturbed implausible triples.}
         \label{fig:distribution_implausible_ts}
     \end{subfigure}
     \hfill
        \caption{Proportion of majority rating across abstractness combinations for attested plausible triples (a) and perturbed implausible triples (b). Blue bars denote a majority of plausible ratings $\in \{4,5\}$, orange bars refer to a majority of implausible ratings $\in \{1,2\}$, and green bars denote a tie with equal numbers of both ratings.}
        \label{fig:majority}
\end{figure*}

\subsection{Exploring the Impact of Abstractness on Plausibility Ratings}
%\paragraph{Does Abstractness Impact Plausibility Ratings?} 
To assess the relation between degrees of abstractness for combinations of words and plausibility on physical and abstract levels, we first examine the proportion of plausibility ratings across triples from each of our 27 abstractness combinations. For this, we calculate majority (50\% or more) ratings for each triple. Whenever a tie, i.e., \textit{full disagreement} is encountered (50:50), both labels are assigned. We present a visualization in Fig.~\ref{fig:majority} where blue bars denote a majority of plausible ratings $\in \{4,5\}$  \textit{plausible}, orange bars refer to a majority of implausible ratings $\in \{1,2\}$, and green bars illustrate ties with equal numbers of both ratings. 

For attested plausible triples, original label and proportional majority rating overlap in all cases. However, we observe three cases in which majority ratings proportions fall below 80\%, namely for the mostly concrete combinations $(c,a,c)$, $(a,c,c)$, and $(c,c,m)$. In contrast, majority rating proportions are highest for the more abstract combinations $(m,a,a)$, $(a,a,a)$, and $(a,c,a)$ with $(m,a,a)$ reaching 100\%. We observe a low average of both ties (3.78) and implausible majority ratings (6.91). 
%@Sabine: Hier würde ich gerne Tripel aus jeder Kategorie angucken und schauen, ob ich da grob mit den Annotation übereinstimmen kann.. bei mehr Zeit hätte ich das gerne von mehr Leuten machen lassen, wäre was für  camera-ready
These observations suggest that (i) implausibility is most likely assigned given more concrete words, inducing higher disagreement among annotators, (ii) plausibility is most likely assigned given more abstract words with abstractness combinations including a concrete word again yielding more implausible majority ratings and ties.

For perturbed implausible triples, the picture looks very different with only one abstractness combination for which original and majority rating proportions overlap, namely $(a,c,c)$. However, we find implausible majority rating proportions $\geq$ 30\% for seven mostly concrete combinations\footnote{$(a,c,c)$, $(a,a,c)$, $(a,m,m)$, $(m,a,c)$, $(m,c,m)$, $(c,a,m)$, and $(c,c,c)$}. In contrast, we observe highest plausible ratings ($\geq$ 80\%) for four highly abstract combinations $(a,a,a)$, $(a,m,a)$, $(m,a,a)$, and $(m,m,a)$. Disagreement is generally higher with the average number of ties (10.3) tripled as compared to attested plausible triples.
%@Sabine: Hier würde ich gerne Tripel aus jeder Kategorie angucken und schauen, ob ich da grob mit den Annotation übereinstimmen kann... bei mehr Zeit hätte ich das gerne von mehr Leuten machen lassen, wäre was für camera-ready
These findings underline the findings for attested plausible triples with (i) implausibility being easier to catch given concrete words, and (ii) plausibility connected to more abstract words.

Based on this exploration, we again find that the majority of human annotators tend to agree on what is plausible, while implausibility seems to be harder to catch and introduces more disagreement. Moreover, assignment \textbf{likelihood of plausibility increases with abstractness} of triple constituents, whereas assignment \textbf{likelihood of implausibility increases with concreteness} of triple constituents  -- no matter the underlying original label.
%\textbf{implausibility is more likely} to be assigned \textbf{given high concreteness} of triple constituents, whereas \textbf{plausibility is more likely} to be assigned \textbf{given high abstractness} of triple constituents -- no matter the underlying original label.

\begin{enumerate}[leftmargin=*]
    \item \textbf{Soft Majority voting}: 4 / 2 classes 
    \begin{itemize}[leftmargin=*]
        \item Classes are assigned based on a 70\% annotator majority for a multi-class $(\{1,2,4,5\}$) or binary (plausible: $\{4,5\}$, implausible: $\{1,2\}$) setup.
        \item In case of no clear majority, both class labels are assigned to reflect conflicting perspectives of annotators.
    \end{itemize}
    %\item \textbf{Median}: 4 / 2 classes 
    %    \begin{itemize}[leftmargin=*]
    %    \item 4 classes: Silver Standard classes correspond to the upper median, i.e. if the median value of ratings is .5 it is rounded up.\footnote{See Table~\ref{apptab:upper_median} lists how often rounding up was performed.} 
    %    \item 2 classes: Silver Standard classes correspond to the median where triples with median $\leq3.9$ are labeled implausible and triples with median $\geq4.0$ are labeled plausible. Here, we  account for the observed skew towards plausibility by moving the threshold towards plausibility. In case of ties, both class labels are assigned.
    %\end{itemize}
    \item \textbf{Distribution}: 4 / 2 classes 
    \begin{itemize}[leftmargin=*]
        \item Class distributions are provided for a multi-class ($\{1,2,4,5\}$) or binary (plausible$\{4,5\}$ and implausible $\{1,2\}$) setup.
    \end{itemize}
     \item \textbf{MACE \cite{hovy-etal-2013-learning}: 4 / 2 classes} 
     \begin{itemize}[leftmargin=*]
         \item 
     \end{itemize}
\end{enumerate}

==> sections/machine_learning_experiments.tex <==
\section{Machine Learning Experiments} \label{sec:ml}

